Open-Source Intelligence for Code Provenance and the Security Patterns that Separate Human and Large-Language-Model Implementations of Common Programming Tasks

Developers now draw code from two very different sources, the accumulated human answers on sites such as Stack Overflow and the output of large language models. We ask two questions about that split. First, can the provenance of a code snippet be recovered from the code itself, and second, do the two sources differ in the security patterns they adopt for the same task. Using only open sources, a public gateway of open-weight language models and the public Stack Overflow API, we build a fully reproducible pipeline that collects real implementations of 31 security-sensitive programming tasks, among them OAuth with PKCE, JWT verification, password hashing, and SQL access, from 9 language models and from human answers, and scores every sample with deterministic security and style detectors. On 528 real samples we train a cross-validated classifier that recovers human versus model provenance with 93 percent accuracy against a 78 percent baseline, and a 7-way classifier that attributes a sample to the specific model that wrote it at 48 percent. We then report where the sources diverge on security, which patterns models adopt more often than the human corpus and which they inherit from it. Running the same tasks in Python, JavaScript, Go, and Java, we find the security divergence holds in every language while the provenance boundary is partly language-specific and does not transfer symmetrically between them. A vulnerability repair case study, in which models are handed insecure code and asked to fix it, finds a 77 percent repair rate across 21 seeds and 12 weakness classes, but a recurring partial-fix failure in which the model removes the insecure pattern without adding the correct defense. The pipeline is data driven, so any new task or language is added as a single specification entry, and a fail-closed checker re-derives every number in this paper from the stored data.

==> sections/listings/cors_config_go_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 58451189 (score 7), cors config go},label={lst:cors_config_go_h}]
// Initialize express middleware
const express = require('express');
const app = express();

// Enable CORS
app.use(function (req, res, next) {
    res.header("Access-Control-Allow-Origin", "*");
    res.header("Access-Control-Allow-Methods", "GET,HEAD,OPTIONS,PO...
    res.header("Access-Control-Allow-Headers", "Origin, X-Requested...
    next();
});
\end{lstlisting}
\end{minipage}


==> sections/listings/cors_config_go_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-nano-30b, cors config go},label={lst:cors_config_go_l}]
package main

import (
    "log"
    "net/http"

    "github.com/gorilla/cors"
)

// CORS configuration   adjust origins, methods, headers, etc. as n...
func main() {
    corsCfg := cors.Config{
        // Allow requests from the frontend's origin.
        AllowOrigins: []string{"https://frontend.example.com"},
        // Permit cookies and Authorization headers.
        AllowCredentials: true,
        // HTTP methods used by the frontend.
        AllowMethods: []string{"GET", "POST", "PUT", "DELETE", "OPT...
        // Custom headers the frontend may send.
        AllowHeaders: []string{"Authorization", "Content-Type"},
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/cors_config_js_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 64729487 (score 22), cors config js},label={lst:cors_config_js_h}]
app.use(
  helmet({
    contentSecurityPolicy: {
      directives: {
        ...helmet.contentSecurityPolicy.getDefaultDirectives(),
        "script-src": ["'self'", "'unsafe-inline'", "example.com"],
      },
    },
  })
);
\end{lstlisting}
\end{minipage}


==> sections/listings/cors_config_js_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-ultra-550b, cors config js},label={lst:cors_config_js_l}]
const express = require('express');
const cors = require('cors');

const app = express();

// Allow requests from specific frontend origin
const corsOptions = {
  origin: 'https://your-frontend-domain.com', // Replace with your ...
  methods: ['GET', 'POST', 'PUT', 'PATCH', 'DELETE', 'OPTIONS'],
  allowedHeaders: ['Content-Type', 'Authorization'],
  credentials: true, // Allow cookies/auth headers
  maxAge: 86400 // Cache preflight for 24 hours
};

app.use(cors(corsOptions));

// Handle preflight requests explicitly (optional, cors() does this)
app.options('*', cors(corsOptions));

// Your routes here
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/file_upload_go_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-nano-30b, file upload go},label={lst:file_upload_go_l}]
package main

import (
    "io"
    "net/http"
    "os"
    "time"
)

// uploadHandler handles POST requests with a multipart/form-data b...
// It expects a single file field named "file" and stores it under the
// directory "./uploads" using a timestamp based name to avoid coll...
func uploadHandler(w http.ResponseWriter, r *http.Request) {
    // Limit upload size to 10 MiB for safety.
    const maxUpload = 10 << 20 // 10 MB
    r.Body = http.MaxBytesReader(w, r.Body, maxUpload)

    // Parse the multipart form (max 1 file, but we can keep the wh...
    if err := r.ParseMultipartForm(32 << 20); err != nil { // 32 MB...
        http.Error(w, "parse form failed", http.StatusInternalServe...
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/file_upload_js_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-nano-30b, file upload js},label={lst:file_upload_js_l}]
// server.js
import express from 'express';
import multer from 'multer';
import fs from 'fs';
import path from 'path';

// Configure storage destination
const storage = multer.diskStorage({
  destination: (req, file, cb) => {
    const uploadPath = path.join('uploads', 'files');
    // Ensure the directory exists
    fs.mkdirSync(uploadPath, { recursive: true });
    cb(null, uploadPath);
  },
  filename: (req, file, cb) => {
    // Use original name with timestamp to avoid collisions
    const unique = `${Date.now()}-${Math.round(Math.random() * 1e9)}`;
    cb(null, `${unique}-${file.originalname}`);
  },
});
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/jwt_verify_go_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 56907478 (score 15), jwt verify go},label={lst:jwt_verify_go_h}]
token, err := jwt.Parse(tokenString, func(token *jwt.Token) (interf...
 if _, ok := token.Method.(*jwt.SigningMethodRS256); !ok {
     return nil, fmt.Errorf("Unexpected signing method: %v", token....
 }
 kid, ok := token.Header["kid"].(string)
 if !ok {
     return nil, errors.New("kid header not found")
 }
 keys := keySet.LookupKeyID(kid);
 if !ok {
     return nil, fmt.Errorf("key with specified kid is not present ...
 }
 var publickey interface{}
 err = keys.Raw(&publickey)
 if err != nil {
     return nil, fmt.Errorf("could not parse pubkey")
 }
 return publickey, nil
\end{lstlisting}
\end{minipage}


==> sections/listings/jwt_verify_go_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM tencent-hy3, jwt verify go},label={lst:jwt_verify_go_l}]
package main

import (
    "net/http"
    "strings"
    "time"

    "github.com/golang-jwt/jwt/v5"
)

// secretKey is used to sign and verify the JWT (HMAC). In producti...
var secretKey = []byte("my-super-secret-key")

// AuthMiddleware verifies the JWT access token from the Authorizat...
func AuthMiddleware(next http.Handler) http.Handler {
    return http.HandlerFunc(func(w http.ResponseWriter, r *http.Req...
        authHeader := r.Header.Get("Authorization")
        if authHeader == "" {
            http.Error(w, "Authorization header required", http.Sta...
            return
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/jwt_verify_js_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 30037296 (score 3), jwt verify js},label={lst:jwt_verify_js_h}]
if (token) {
    // We use `return` only to stop further processing of the middl...
    // we don't actually care about the return value from `jwt.veri...
    return jwt.verify(token, superSecret, function(err, decoded) {
        if (err) {
            return next(err);
        }
        // if everything is good, save to request for use in other ...
        else {
          req.decoded = decoded;
          next();
        }
    });
}
\end{lstlisting}
\end{minipage}


==> sections/listings/jwt_verify_js_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-small-4-119b, jwt verify js},label={lst:jwt_verify_js_l}]
const jwt = require('jsonwebtoken');
const { promisify } = require('util');

// Promisify jwt.verify for async/await usage
const verifyToken = promisify(jwt.verify);

// Middleware to authenticate API requests using JWT
async function authenticateToken(req, res, next) {
  // Extract token from Authorization header (Bearer scheme)
  const authHeader = req.headers['authorization'];
  const token = authHeader && authHeader.split(' ')[1]; // Format: ...

  if (!token) {
    return res.status(401).json({ error: 'Access token required' });
  }

  try {
    // Verify token using secret key (replace with your actual secret)
    const decoded = await verifyToken(token, process.env.JWT_SECRET...
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/landing_page_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-small-4-119b, landing page},label={lst:landing_page_l}]
<!DOCTYPE html>
<html lang="en">
<head>
    <meta charset="UTF-8">
    <meta name="viewport" content="width=device-width, initial-scal...
    <title>Product Landing Page</title>
    <style>
        /* Reset and base styles */
        * {
            margin: 0;
            padding: 0;
            box-sizing: border-box;
        }

        body {
            font-family: 'Arial', sans-serif;
            line-height: 1.6;
            color: #333;
        }
<!-- ... -->
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth2_django_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 61707725 (score 6), oauth2 django},label={lst:oauth2_django_h}]
from allauth.socialaccount.providers.google.views import GoogleOAut...
from allauth.socialaccount.providers.oauth2.client import OAuth2Client
from rest_auth.registration.views import SocialLoginView


class GoogleLogin(SocialLoginView):
    adapter_class = GoogleOAuth2Adapter
    client_class = OAuth2Client
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth2_django_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM codestral, oauth2 django},label={lst:oauth2_django_l}]
# settings.py

# Add to INSTALLED_APPS
INSTALLED_APPS = [
    ...
    'social_django',
    ...
]

# Add to MIDDLEWARE
MIDDLEWARE = [
    ...
    'social_django.middleware.SocialAuthExceptionMiddleware',
    ...
]

# Add to TEMPLATES
TEMPLATES = [
    {
        ...
# ...
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth2_express_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 50504098 (score 3), oauth2 express},label={lst:oauth2_express_h}]
import React, { Component, Fragment } from 'react'
import { BrowserRouter as Router, Route, Switch } from 'react-route...

import PrivateRoute from '../util/PrivateRoute'

// Components
import Navbar from './layout/Navbar'

import Landing from './Landing'
import SocialLogin from './SocialLogin'
import Dashboard from './Dashboard'

class App extends Component {
    render() {
        return (
            <Router>
                <Fragment>
                    <Navbar /><br />

                    <Route exact path="/" component={Landing} />
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth2_express_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-nano-30b, oauth2 express},label={lst:oauth2_express_l}]
// app.js
import express from "express";
import session from "express-session";
import passport from "passport";
import { Strategy as GoogleStrategy } from "passport-google-oauth20";

const app = express();
const PORT = 3000;

// ---------- Middleware ----------
app.use(express.urlencoded({ extended: true }));
app.use(express.json());

// Session support (required for Passport)
app.use(
  session({
    secret: "your-secret-key",
    resave: false,
    saveUninitialized: false,
    cookie: { maxAge: 86400000 }, // 1 day
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth2_spring_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 70259040 (score 10), oauth2 spring},label={lst:oauth2_spring_h}]
@Configuration
public class Tenant1SecurityConfiguration extends WebSecurityConfig...

    @Override
    protected void configure(HttpSecurity http) throws Exception {
        http
                .csrf().disable()
                .authorizeRequests()
                .antMatchers("/login**").permitAll()
                .antMatchers("/manage/**").permitAll()
                .antMatchers("/api/auth-info").permitAll()
                .antMatchers("/api/**").authenticated()
                .antMatchers("/management/health").permitAll()
                .antMatchers("/management/info").permitAll()
                .antMatchers("/management/prometheus").permitAll()
                .antMatchers("/management/**").hasAuthority("ADMIN")
                .antMatchers("/tenant1/**").authenticated()
                .and()
                .oauth2Login()
                .and()
# ...
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth2_spring_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-small-4-119b, oauth2 spring},label={lst:oauth2_spring_l}]
// OAuth2LoginConfig.java
package com.example.demo.config;

import org.springframework.context.annotation.Bean;
import org.springframework.context.annotation.Configuration;
import org.springframework.security.config.annotation.web.builders....
import org.springframework.security.config.annotation.web.configura...
import org.springframework.security.web.SecurityFilterChain;

@Configuration
@EnableWebSecurity
public class OAuth2LoginConfig {

    @Bean
    public SecurityFilterChain securityFilterChain(HttpSecurity htt...
        http
            .authorizeHttpRequests(authorize -> authorize
                .requestMatchers("/", "/login**", "/error**").permi...
                .anyRequest().authenticated()
            )
# ...
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth_pkce_go_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-nano-30b, oauth pkce go},label={lst:oauth_pkce_go_l}]
package main

import (
    "crypto/rand"
    "encoding/base64"
    "encoding/json"
    "flag"
    "fmt"
    "io"
    "net/http"
    "net/url"
    "strings"
    "log"
)

// Config holds OAuth client information and endpoints.
type Config struct {
    ClientID     string // required
    RedirectURL  string // must be registered in the provider console
    AuthURL      string // e.g. https://provider.com/oauth2/auth
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/oauth_pkce_js_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-large-3-675b, oauth pkce js},label={lst:oauth_pkce_js_l}]
const express = require('express');
const crypto = require('crypto');
const axios = require('axios');
const session = require('express-session');
const querystring = require('querystring');

// Configuration - replace with your OAuth provider's details
const config = {
  clientId: 'your-client-id',
  clientSecret: 'your-client-secret', // Only needed if confidentia...
  redirectUri: 'http://localhost:3000/callback',
  authorizationEndpoint: 'https://oauth-provider.com/authorize',
  tokenEndpoint: 'https://oauth-provider.com/token',
  scope: 'openid profile email',
  sessionSecret: 'your-session-secret'
};

const app = express();

// Middleware
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/path_serve_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 60152031 (score 2), path serve},label={lst:path_serve_h}]
hook = MsSqlHook(mssql_conn_id="detbds")
with hook.get_conn() as conn:
    conn.autocommit = True
    cursor = conn.cursor()
\end{lstlisting}
\end{minipage}


==> sections/listings/path_serve_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM north-mini-code, path serve},label={lst:path_serve_l}]
from flask import Flask, send_from_directory, abort
import os

app = Flask(__name__)

# Define the directory from which files will be served
BASE_DIR = os.path.abspath("files")

@app.route('/files/<filename>')
def get_file(filename):
    """
    Serves a file from the BASE_DIR directory based on the provided...
    Includes security checks to prevent directory traversal attacks.
    """
    # Sanitize the filename to prevent directory traversal
    safe_filename = os.path.basename(filename)
    file_path = os.path.join(BASE_DIR, safe_filename)

    # Check if the file exists and is a file (not a directory)
    if not os.path.isfile(file_path):
# ...
\end{lstlisting}
\end{minipage}


==> sections/listings/secrets_env_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 49812929 (score 29), secrets env},label={lst:secrets_env_h}]
AIRFLOW__WEBSERVER__BASE_URL="https://your_ip_or_domain:port"
\end{lstlisting}
\end{minipage}


==> sections/listings/secrets_env_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-small-4-119b, secrets env},label={lst:secrets_env_l}]
import os
from typing import Optional
import requests

def load_api_key(env_var: str = "API_KEY") -> Optional[str]:
    """Load API key from environment variable."""
    return os.getenv(env_var)

def make_api_request(api_key: str, endpoint: str, params: dict = No...
    """Make a request to a third-party API using the provided key."""
    headers = {"Authorization": f"Bearer {api_key}"}
    response = requests.get(endpoint, headers=headers, params=params)
    response.raise_for_status()  # Raise exception for HTTP errors
    return response.json()

# Example usage
if __name__ == "__main__":
    api_key = load_api_key()
    if not api_key:
        raise ValueError("API key not found in environment variables")
# ...
\end{lstlisting}
\end{minipage}


==> sections/listings/session_cookie_go_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-small-4-119b, session cookie go},label={lst:session_cookie_go_l}]
package main

import (
    "net/http"
    "time"
)

// SetSessionCookie sets a session cookie for a logged-in user
func SetSessionCookie(w http.ResponseWriter, userID string) {
    // Create a secure, HTTP-only cookie with a session token
    cookie := &http.Cookie{
        Name:     "session_token",
        Value:    userID, // In production, use a secure token instead
        Expires:  time.Now().Add(24 * time.Hour), // 24-hour expira...
        HttpOnly: true, // Prevents JavaScript access
        Secure:   true, // Only send over HTTPS
        SameSite: http.SameSiteStrictMode, // CSRF protection
        Path:     "/", // Available across the entire domain
    }
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/session_cookie_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 22930708 (score 9), session cookie},label={lst:session_cookie_h}]
credentials = AccessTokenCredentials(session['credentials'], 'user-...
\end{lstlisting}
\end{minipage}


==> sections/listings/session_cookie_js_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 73847443 (score 3), session cookie js},label={lst:session_cookie_js_h}]
// if user is not logged-in redirect back to login page
app.use(function(req, res, next) {
   if (req.session.user == null){
   res.redirect('http://localhost:3000/login');
   }   else {
    next();
   }
});
\end{lstlisting}
\end{minipage}


==> sections/listings/session_cookie_js_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-large-3-675b, session cookie js},label={lst:session_cookie_js_l}]
const express = require('express');
const cookieSession = require('cookie-session');
const app = express();

// Configure cookie session middleware
app.use(cookieSession({
  name: 'session', // Name of the cookie
  keys: ['your-secret-key-1', 'your-secret-key-2'], // Keys for sig...
  maxAge: 24 * 60 * 60 * 1000, // Session duration in milliseconds ...
  httpOnly: true, // Prevent client-side JS access
  secure: process.env.NODE_ENV === 'production', // Only send over ...
  sameSite: 'lax' // Protection against CSRF
}));

// Example route to set session cookie on login
app.post('/login', (req, res) => {
  // Authenticate user (this is just an example)
  const { username, password } = req.body;
  if (username === 'admin' && password === 'password') { // Replace...
    req.session.user = { id: 1, username: 'admin' }; // Set user da...
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/session_cookie_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-small-4-119b, session cookie},label={lst:session_cookie_l}]
from flask import Flask, make_response, session
from datetime import timedelta

app = Flask(__name__)
app.secret_key = 'your-secret-key-here'  # Required for session sec...

@app.route('/login', methods=['POST'])
def login():
    # Authenticate user (example: check credentials)
    username = request.form.get('username')
    password = request.form.get('password')
    if authenticate_user(username, password):  # Replace with your ...
        # Create session cookie with 1-hour expiration
        response = make_response("Login successful")
        session.permanent = True  # Makes session cookie persistent
        session['username'] = username  # Store user data in session
        response.set_cookie(
            'session_id',
            value=session.get('_id'),  # Flask's session ID
            max_age=int(timedelta(hours=1).total_seconds()),
# ...
\end{lstlisting}
\end{minipage}


==> sections/listings/spring_jpa_query_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 57165352 (score 18), spring jpa query},label={lst:spring_jpa_query_h}]
EmbeddedDataSourceBeanFactoryPostProcessor : Replacing 'dataSource'...
\end{lstlisting}
\end{minipage}


==> sections/listings/spring_jpa_query_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM nemotron-3-ultra-550b, spring jpa query},label={lst:spring_jpa_query_l}]
import org.springframework.data.jpa.repository.JpaRepository;
import org.springframework.data.jpa.repository.Query;
import org.springframework.data.repository.query.Param;
import org.springframework.stereotype.Repository;
import java.util.Optional;

@Repository
public interface UserRepository extends JpaRepository<User, Long> {

    // Derived query method (Spring Data JPA generates SQL from met...
    Optional<User> findByName(String name);

    // Explicit JPQL query (useful for complex logic or custom naming)
    @Query("SELECT u FROM User u WHERE u.name = :name")
    Optional<User> findByNameExplicit(@Param("name") String name);

    // Native SQL query (if you need database-specific features)
    @Query(value = "SELECT * FROM users WHERE name = :name", native...
    Optional<User> findByNameNative(@Param("name") String name);
}
\end{lstlisting}
\end{minipage}


==> sections/listings/sql_query_go_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM codestral, sql query go},label={lst:sql_query_go_l}]
package main

import (
    "database/sql"
    "fmt"
    "log"
    "os"

    _ "github.com/lib/pq" // PostgreSQL driver
)

// User represents a user in the database
type User struct {
    ID       int
    Username string
    Email    string
}

func main() {
    // Get the username from command line arguments
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/sql_query_js_llm.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={LLM mistral-large-3-675b, sql query js},label={lst:sql_query_js_l}]
const { createPool } = require('mysql2/promise'); // Using mysql2 f...

// Database configuration - adjust these values to match your envir...
const dbConfig = {
  host: 'localhost',
  user: 'your_db_user',
  password: 'your_db_password',
  database: 'your_db_name',
  waitForConnections: true,
  connectionLimit: 10,
  queueLimit: 0
};

const pool = createPool(dbConfig);

/**
 * Looks up a user by username in the database
 * @param {string} username - The username to search for
 * @returns {Promise<Object|null>} The user object if found, null o...
 * @throws {Error} If there's a database error
// ...
\end{lstlisting}
\end{minipage}


==> sections/listings/ssrf_fetch_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 66619020 (score 3), ssrf fetch},label={lst:ssrf_fetch_h}]
if request.method=='POST':
    if 'add_note_button' in request.form:
        # do things
    elif 'remove_note_button' in request.form:
        # do things
\end{lstlisting}
\end{minipage}


==> sections/listings/xss_escape_human.tex <==
% AUTO
\noindent\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={Human SO answer 44060306 (score 21), xss escape},label={lst:xss_escape_h}]
flask.url_for('user', nickname=post.author.nickname)
\end{lstlisting}
\end{minipage}

